Blind Deinterleaving of Signals in Time Series with Self-attention Based Soft Min-cost Flow Learning

We propose an end-to-end learning approach to address deinterleaving of patterns in time series, in particular, radar signals. We link signal clustering problem to min-cost flow as an equivalent problem once the proper costs exist. We formulate a bi-level optimization problem involving min-cost flow as a sub-problem to learn such costs from the supervised training data. We then approximate the lower level optimization problem by self-attention based neural networks and provide a trainable framework that clusters the patterns in the input as the distinct flows. We evaluate our method with extensive experiments on a large dataset with several challenging scenarios to show the efficiency.

==> ICASSP 2021/authors.tex <==
\name{O\u{g}ul Can$^\dagger$ \qquad Yeti Z. G\"{u}rb\"{u}z$^\dagger$ \qquad Berkin Y{\i}ld{\i}r{\i}m$^\ast$ \qquad  A. Ayd{\i}n Alatan$^\dagger$\thanks{This study is supported by ASELSAN A. Ş.}}

\address{$^\dagger$Dept. of Elect. Elec. Eng. \& Center for Image Analysis (OGAM)\\
Middle East Technical University, Ankara, Turkey\\
$^\ast$ASELSAN A. Ş., Ankara, Turkey}
%    $^{\star}$ Center for Image Analysis(OGAM), Middle East Technical University, Ankara, Turkey}

%    $^{\star}$ Center for Image Analysis(OGAM), Middle East Technical University, Ankara, Turkey}
%
% For example:
% ------------
%\address{School\\
%	Department\\
%	Address}
%
% Two addresses (uncomment and modify for two-address case).
% ----------------------------------------------------------
%\twoauthors
%  {Yeti Z. G\"{u}rb\"{u}z$^{\dagger}$ \qquad O\u{g}ul Can$^{\star}$\thanks{This study is supported by ESEN System Integration.}}
%	{$^{\dagger}$Dept. of Elect. and Elec. Eng.\\
%	Middle East Technical University\\
%	Ankara, Turkey}
%  {A. Ayd{\i}n Alatan$^{\dagger \star}$}
%	{$^{\star}$Center for Image Analysis (OGAM)\\
%	Middle East Technical University \\
%	Ankara, Turkey}



%
% For example:
% ------------
%\address{School\\
%	Department\\
%	Address}
%
% Two addresses (uncomment and modify for two-address case).
% ----------------------------------------------------------
%\twoauthors
%  {A. Author-one, B. Author-two\sthanks{Thanks to XYZ agency for funding.}}
%	{School A-B\\
%	Department A-B\\
%	Address A-B}
%  {C. Author-three, D. Author-four\sthanks{The fourth author performed the work
%	while at ...}}
%	{School C-D\\
%	Department C-D\\
%	Address C-D}
%

==> ICASSP 2021/definitions.tex <==
% Example definitions.
% --------------------
%\def\x{{\mathbf x}}
%\def\L{{\cal L}}

\newcommand{\vect}[1]{\boldsymbol{#1}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\tr}{tr}
%\DeclareMathOperator{\Exp}{\mathbb{E}}
\newcommand{\KL}[2]{\ensuremath{\operatorname{KL}\left[{#1} \parallel {#2} \right]}}
\newcommand{\E}[2]{\ensuremath{\operatorname{\mathbb{E}}_{#2}\left[ {#1} \right]}}
\newcommand{\TD}[3]{\ensuremath{\operatorname{TD}_{#2}^{#3}\left( {#1} \right)}}
\newcommand{\WD}[3]{\ensuremath{\operatorname{WD}_{#2}^{#3}\left( {#1} \right)}}
\newcommand{\diag}[1]{\ensuremath{\operatorname{diag}( {#1} )}}
\newcommand{\1}{\ensuremath{\vect{\mathbbm{1}}}}
\newcommand{\ind}[1]{\ensuremath{\mathbbm{1}_{#1}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\T}{\ensuremath{^\intercal}}
\newcommand{\grad}{\ensuremath{\nabla}}
\def\smallint{\begingroup\textstyle \int\endgroup}

\newcommand{\ie}{\textit{i}.\textit{e}., }
\newcommand{\eg}{\textit{e}.\textit{g}. }

%\newenvironment{theorem}[1]{\par\noindent\underline{Theorem:}\space#1}{}
%\newenvironment{proof}[1]{\par\noindent\underline{Proof:}\space#1}{\hfill $\blacksquare$}

\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[proposition]
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]

\numberwithin{equation}{section}


==> ICASSP 2021/figures/fig_the_figure_1.tex <==
% Below is an example of how to insert images. Delete the ``\vspace'' line,
% uncomment the preceding line ``\centerline...'' and replace ``imageX.ps''
% with a suitable PostScript file name.
% -------------------------------------------------------------------------
\begin{figure}[t]
  \centering
  \centerline{\includegraphics[width=.95\linewidth]{figures/the_figure_1.png}}
  \caption{Overview of the Soft Min-cost Flow Framework}
	\label{fig:the_figure_1}
  \end{figure}

	
%
%\end{wrapfigure}


==> ICASSP 2021/figures/pri_fig.tex <==
% Below is an example of how to insert images. Delete the ``\vspace'' line,
% uncomment the preceding line ``\centerline...'' and replace ``imageX.ps''
% with a suitable PostScript file name.
% -------------------------------------------------------------------------
\begin{figure}[t]
  \centering
  \centerline{\includegraphics[width=\linewidth]{figures/pri.png}}
  \caption{PRI types. (a) 500 $\mu$s constant PRI. (b) 500 $\mu$s jitter PRI with +/-10\% jitter. (c) [500, 400, 600] $\mu$s constant stagger PRI with 3 stagger levels. (d) [400, 500, 600] $\mu$s random stagger PRI with 3 stagger levels. (e) [600, 400, 500] $\mu$s switch\&dwell PRI with [5, 7, 3] dwells and 3 switches.}
	\label{fig:pri_types}
  \end{figure}

	
%
%\end{wrapfigure}

==> ICASSP 2021/figures/table_performance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[!t]
\centering
\caption{Comparison with the existing and baseline methods for the deinterleaving task. The best results are indicated in bold.}
\label{tab:results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c|}
Dataset -  \text{$Acc_{link}$} / \text{$Acc_{nor}$} / \text{$V_{1-m}$} & CDIF & SDIF & PRIT & Baseline + Greedy & Baseline + LP & SMCF + Greedy & SMCF + LP \\ \hline
Validation - Case 1 & 0.841 / 0.605 / 0.000 & 0.850 / 0.614 / 0.000 & 0.982 / 0.631 / 0.000 & 0.975 / 0.940 / 0.013 & 0.963 / 0.966 / 0.000 & \textbf{0.991} / \textbf{0.998} / \textbf{0.001} & \textbf{0.991} / \textbf{0.998} / 0.000 \\
Validation - Case 2 & 0.519 / 0.312 / 0.000 & 0.518 / 0.309 / 0.000 & 0.631 / 0.538 / 0.000 & 0.894 / 0.758 / 0.201 & 0.885 / 0.764 / 0.000 & \textbf{0.945} / \textbf{0.996} / \textbf{0.004} & 0.943 / 0.994 / 0.000 \\
Validation - Case 3 & 0.352 / 0.154 / 0.000 & 0.362 / 0.157 / 0.000 & 0.579 / 0.437 / 0.000 & 0.858 / 0.623 / 7.477 & 0.856 / 0.627 / 0.000 & 0.912 / 0.950 / \textbf{0.025} & \textbf{0.915} / \textbf{0.954} / 0.000 \\
Validation - Case 4 & 0.679 / 0.480 / 0.000 & 0.683 / 0.481 / 0.000 & 0.768 / 0.545 / 0.000 & 0.956 / 0.977 / 0.011 & 0.955 / 0.977 / 0.000 & \textbf{0.991} / \textbf{0.999} / \textbf{0.002} & 0.990 / 0.998 / 0.000 \\
Validation - Case 5 & 0.548 / 0.370 / 0.000 & 0.550 / 0.364 / 0.000 & 0.642 / 0.496 / 0.000 & 0.901 / 0.836 / 2.736 & 0.900 / 0.841 / 0.000 & \textbf{0.929} / \textbf{0.975} / \textbf{0.015} & \textbf{0.929 }/ \textbf{0.975} / 0.000 \\
Test & 0.304 / 0.147 / 0.000 & 0.311 / 0.148 / 0.000 & 0.564 / 0.436 / 0.000 & 0.842 / 0.539 / 11.943 & 0.823 / 0.555 / 0.000 & \textbf{0.903} / 0.883 / \textbf{0.098} & 0.898 / \textbf{0.886} / 0.000
\end{tabular}%
}
\end{table*}

==> ICASSP 2021/packages.tex <==
\usepackage{import}
\usepackage{spconf}

\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{commath}
\usepackage{mathrsfs}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{bbm}
\usepackage{fancyhdr}
\usepackage{cancel}

\usepackage{algorithm}
\usepackage{algpseudocode}

\usepackage{graphicx}
\usepackage{epsfig}
\usepackage[utf8]{inputenc}
\usepackage{tabularx}
\usepackage{booktabs, multicol, multirow}
\usepackage[table,xcdraw]{xcolor}

\usepackage{caption}
\usepackage{subcaption}

\usepackage{appendix}

\usepackage{cite}
%\usepackage{hyperref}
\usepackage{url}
%\usepackage{breqn}






